Versatile Video Coding Standard: A Review from Coding Tools to Consumers Deployment

The amount of video content and the number of applications based on multimedia information increase each day. The development of new video coding standards is a challenge to increase the compression rate and other important features with a reasonable increase in the computational load. Video Experts Team (JVET) of ITU-T and the JCT group within ISO/IEC have worked together to standardize the Versatile Video Coding, approved finally in July 2020 as ITU-T H.266 | MPEG-I - Part 3 (ISO/IEC 23090-3) standard. This paper overviews some interesting consumer electronic use cases, the compression tools described in the standard, the current available real time implementations and the first industrial trials done with this standard.

==> Fig/dualtree.tex <==

    \centering
    \begin{tabular}{ccc}
    \multicolumn{3}{c}{\includegraphics[scale=0.73]{Fig/decoded_yuv.png}}
    
    \\ 
    
    \multicolumn{3}{c}{(a) $YC_bC_r$}
    
    \\
    & & 
    \\
    
    \includegraphics[scale=0.43]{Fig/partitioning_y.png}
    &  
    \includegraphics[scale=0.43]{Fig/partitioning_cb.png}
    & 
    \includegraphics[scale=0.43]{Fig/partitioning_cr.png}
    \\ 
    (b) $Y$ & (c) $C_b$ & (d) $C_r$  
    \end{tabular}
    

